Vibrationally excited HCN transitions in circumstellar envelopes of carbon-rich AGB stars

Context. HCN is the most abundant molecule after H$_{2}$ and CO in the circumstellar envelopes (CSEs) of carbon-rich asymptotic giant branch (AGB) stars. Its rotational lines within vibrationally excited states are exceptional tracers of the innermost region of C-rich CSEs. Aims. We aim to constrain the physical conditions of CSEs of C-rich stars using thermal lines of the HCN molecule. Additionally, we also search for new HCN masers and probe the temporal variations for HCN masers, which should shed light on their pumping mechanisms. Methods. We observed 16 C-rich AGB stars in various HCN rotational transitions within the ground and 12 vibrationally excited states with the APEX 12 m submillimeter telescope. Results. We detect 68 vibrationally excited HCN lines from 13 C-rich stars, including 39 thermal transitions and 29 maser lines, which suggests that vibrationally excited HCN lines are ubiquitous in C-rich stars. Population diagrams constructed, for two objects from the sample, for thermal transitions from different vibrationally excited states give excitation temperature around 800-900 K, confirming that they arise from the hot innermost regions of CSEs (i.e., r<20$R_{*}$). Among the detected masers, 23 are newly detected, and the results expand the total number of known HCN masers lines toward C-rich stars by 47%. In particular, the J=2-1 (0, 3$^{1e}$, 0), J=3-2 (0, 2, 0), J=4-3 (0, 1$^{1f}$, 0) masers are detected in an astronomical source for the first time. Our observations confirm temporal variations of the 2-1 (0, 1$^{1e}$, 0) maser on a timescale of a few years. Our analysis of the data suggests that all detected HCN masers are unsaturated. A gas kinetic temperature of ${\gtrsim}$700K and an H$_{2}$ number density of >10$^{8}$cm$^{-3}$ are required to excite the HCN masers. In some ways, HCN masers in C-rich stars might be regarded as an analogy of SiO masers in O-rich stars.

==> longtable-bak.tex <==
%\begin{landscape}
\onecolumn  
\begin{center}

%\newpage
\begin{longtable}{cccccc}%{ccccccp{5.5cm}}
% \begin{table*}

%\centering
\caption{\textbf {Catalogue of HCN maser detections in the CSEs of 31 stars till date.}}
\label{maser_catalogue}
\\ \hline 
%\label{maser_catalogue}

\hline
%\multicolumn{6}{ c }{Begin of Table}\\
\hline
Source name &  $\nu$ (MHz) & $J$ & $(\nu_{1}, \nu_{2}, \nu_{3})$ & Publication & Notes\\ 
%\hline
%\endfirsthead


%\multicolumn{6}{c}{Continuation of Table \ref{maser_catalogue}}\\
%\hline
%Source name &  $\nu$ (MHz) & J & $(\nu_{1}, \nu_{2}, \nu_{3})$ & Publication & Notes\\ 
%\hline
%\endhead

%\hline
%\endfoot

%\hline
%\multicolumn{6}{ c }{End of Table}\\
\hline
%\endlastfoot
%\hline
AFGL 2513 & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\* 
%\hline
Al Vol & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
Al Vol & 178136.477 & 2 $-$ 1 & (0,1$^{1f}$,0) & \citet{2018AA...613A..49M} & \\*
%\hline
CIT6   & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{guilloteau1987new}& \\*
CIT6 & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) &\citet{2018AA...613A..49M} &\\*
CIT6 & 178136.477 & 2 $-$ 1 & (0,1$^{1f}$,0) & \citet{2018AA...613A..49M} &\\*
CIT6$^b$  & 804750.9 & 9 $-$ 8 & (0, 4, 0) & \citet{schilke..menten2003ApJ...583..446S} & \\*
CIT6      & 890761.0 & 10 $-$ 9 & (1,1$^{1}$,0) $-$ (0, 4, 0) & \citet{schilke..menten2003ApJ...583..446S} & \\*
%\hline
CRL 3068  & 177238.656 & 2 $-$ 1 & (0,1$^{1e}$,0) & This work &\\*
CRL 3068  & 356255.568 & 4 $-$ 3 & (0, 1$^{1f}$, 0) &This work & \\*
%\hline
CQ Pyx & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
CQ Pyx & 178136.477 & 2 $-$ 1 & (0,1$^{1f}$,0) & \citet{2018AA...613A..49M} & \\*
%\hline
FX Ser & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
II Lup & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
II Lup & 356255.568 & 4 $-$ 3 & (0, 1$^{1f}$, 0) &This work & \\*
%\hline
IRAS1758-1744 & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
IRC+10216 & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1986first} & \\*
IRC+10216 & 177238.710 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{lucas1989cerni..discovery} &  \\*
IRC+10216 & 177238.655 & 2 $-$ 1 & (0,1$^{1f}$,0) & \citet{2018AA...613A..49M} & \\*
IRC+10216 & 356255.568 & 4 $-$ 3 & (0, 1$^{1f}$, 0) &This work & \\*
IRC+10216 & 804750.9 & 9 $-$ 8 & (0, 4, 0) & \citet{schilke..mehringer..menten2000ApJ...528L..37S} & \\*
IRC+10216 & 890761.0 & 10 $-$ 9 & (1,1$^{1}$,0) $-$ (0, 4, 0) & \citet{schilke..menten2003ApJ...583..446S} & \\*
%\hline
IRC+20370 & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
IRC+20370 & 265852.709 & 3 $-$ 2 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
IRC+30374 & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
IRC+50096 & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
RAFGL 4211 & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
RAFGL 4211 & 266539.980 & 3 $-$ 2 & (0, 3$^{1e}$, 0) & This work& \\*
RAFGL 4211 & 267243.150 & 3 $-$ 2 & (0, 2, 0)  &This work &\\*
RAFGL 4211 & 354460.435 & 4 $-$ 3 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
R For  & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
%\hline
R Lep  & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
R Lep  & 265852.709 & 3 $-$ 2 & (0,1$^{1e}$,0) & \citet{Bieging_2001} & \\*
%\hline
R Scl  & 265852.709 & 3 $-$ 2 & (0,1$^{1e}$,0) & \citet{Bieging_2001} & \\*
%\hline
RV Aqr & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
RV Aqr & 178136.478 & 2 $-$ 1 & (0, 1$^{1f}$, 0) & This work& \\*
RV Aqr & 265852.709 & 3 $-$ 2 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
R Vol & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
R Vol & 178136.478 & 2 $-$ 1 & (0, 1$^{1f}$, 0) & This work& \\*
R Vol & 265852.709 & 3 $-$ 2 & (0, 1$^{1e}$, 0) & This work& \\*
R Vol & 354460.435 & 4 $-$ 3 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
S Aur & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
S Cep & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
T Dra & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{lucas1988new} & \\*
%\hline
UU Aur & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{izumiura..1995ApJ...440..728I} & First published in Izumiura's PhD thesis \\*
%\hline
V636 Mon & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
V 384 Per & 265852.709 & 3 $-$ 2 & (0,1$^{1e}$,0) & \citet{Bieging_2001} & \\*
%\hline
V Aql & 265852.709 & 3 $-$ 2 & (0, 1$^{1e}$, 0) & This work& \\*
%\hline
V Cyg$^a$ & 265852.709 & 3 $-$ 2 & (0,1$^{1e}$,0) & \citet{Bieging_2001} & \\*
%\hline
V Hya & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\*
%\hline
W Ori & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{olofsson1993bstudy} & \\*
W Ori & 177238.656 & 2 $-$ 1 & (0, 1$^{1e}$, 0) & This work& \\*
W Ori & 265852.709 & 3 $-$ 2 & (0, 1$^{1e}$, 0) & This work& \\*
W Ori & 267199.283 & 3 $-$ 2 & (0, 1$^{1f}$, 0) & This work& \\*
W Ori & 354460.435 & 4 $-$ 3 & (0, 1$^{1e}$, 0) & This work& \\
%\hline
X Vel & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{olofsson1993bstudy} & \\
X Vel & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M}& \\
%\hline
X TrA & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{olofsson1993bstudy} & \\
X TrA & 177238.655 & 2 $-$ 1 & (0,1$^{1e}$,0) & \citet{2018AA...613A..49M} & \\
%\hline
Y CVn & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{izumiura1987} & Spike emission of maser origin\\
Y CVn & 265852.709 & 3 $-$ 2 & (0,1$^{1e}$,0) & \citet{Bieging_2001} & \\
Y CVn & 890761.0   & 10 $-$ 9 & (1,1$^{1}$,0) $-$ (0, 4, 0) & \citet{schilke..menten2003ApJ...583..446S} & \\
%\hline
Y Tau & 89087.7 & 1 $-$ 0& (0, 2, 0) & \citet{izumiura..1995ApJ...440..728I} & First published in Izumiura's PhD thesis \\
\hline


\caption{Catalogue HCN masers detected in AGB stars until now. $^a$ first discovered by \citet{bieging2000vcygsubmillimeter}, and then confirmed by \citet{Bieging_2001}. $^b$ A tentative detection by \citet{schilke..menten2003ApJ...583..446S}.}
%\end{tabular}
%\tablefoot{$^a$ first discovered by \citet{bieging2000vcygsubmillimeter}, and then confirmed by \citet{Bieging_2001}. $^b$ A tentative detection by \citet{schilke..menten2003ApJ...583..446S}.}
%\end{table*}
%\end{landscape}

\end{longtable}
\end{center}
%\clearpage
\twocolumn

